Learning Stable Vector Fields on Lie Groups

Learning robot motions from demonstration requires models able to specify vector fields for the full robot pose when the task is defined in operational space. Recent advances in reactive motion generation have shown that learning adaptive, reactive, smooth, and stable vector fields is possible. However, these approaches define vector fields on a flat Euclidean manifold, while representing vector fields for orientations requires modeling the dynamics in non-Euclidean manifolds, such as Lie Groups. In this paper, we present a novel vector field model that can guarantee most of the properties of previous approaches i.e., stability, smoothness, and reactivity beyond the Euclidean space. In the experimental evaluation, we show the performance of our proposed vector field model to learn stable vector fields for full robot poses as SE(2) and SE(3) in both simulated and real robotics tasks.

==> algorithms/algorithm_msvf.tex <==
\begin{algorithm}
    \small
	\SetKwInOut{Input}{Given}
	\Input{$\vx$: Current  robot state in the manifold $\gM$\;
	    $\vx_H$: Origin in $\gM$\;
		$\textrm{LogMap}$: Map to the Tangent Space at the origin\;
		$\phi_{\theta 0}, \dots, \phi_{\theta K}$: Bounded \& smooth Piecewise-Linear \gls{inn} \;
		$\gamma$: Map from Tangent Space at $\vx_H$ to $\gC^n$\;
		$\textrm{FrameChange}$: Adjoint Map for Lie Groups/Map between Tangent Space in $\gS^n$ \;
		$g$: Latent stable vector field}
	\BlankLine
	$\hat{\vx} = \textrm{LogMap}(\vx, \vx_H)$\tcp*{Map to Tangent Space}
	$\hat{\vz} = \gamma^{-1} \circ \phi_{\theta k} \circ \dots \circ \phi_{\theta 0}\circ \gamma (\hat{\vx})$\tcc*{Map to the Latent Tangent Space}
	$\d \vz = g(\hat{\vz})$\tcp*{Compute velocity in the latent space}
	$\mJ^{\dagger} = \textrm{pinv}(\frac{\partial \hat{\vz}}{\partial \hat{\vx}})$\tcp*{Compute Jacobian pseudoinverse}
	$\mA = \textrm{FrameChange}(\vx_H, \vx)$\;
	$\d \vx = \mA \mJ^{\dagger} \d \vz$\;
	\KwRet{$\d \vx$}\;
	
	\caption{Manifold Stable Vector Fields \label{alg:m_svf}}
	\label{alg:svf_manifold}
\end{algorithm}


==> tables/manifold_details.tex <==
\begin{tabular}{ c | c | c | c | c } 
	\hline
	Manifold & $\hat{U}_{\gM}$ & LogMap & ExpMap & $\gamma$\\
	\hline
	$\gS^2$ & $\gB_{\pi}^2:\{ \vx\in \RR^2 \,,\,  |\vx| \leq \pi \} $ & 
	$\begin{aligned}
    	\rho = \arctan\left(\frac{\sqrt{x^2 + y^2}}{z}\right) \quad ,& \quad \theta = \arctan\left(\frac{y}{x}\right) \\
    	 \hat{x} = \rho \cos(\theta) \quad ,& \quad  \hat{y} = \rho \sin(\theta)
	\end{aligned}$
	& 	$\begin{aligned}
	    \rho = \sqrt{\hat{x}^2 + \hat{y}^2} \quad ,& \quad
	    \theta = \arctan( \hat{y}/  \hat{x}) \\
	    x = \cos(\theta) \sin(\rho) \quad,\quad y &= \sin(\theta) \sin(\rho)\quad,\quad z = \cos(\rho)\\
	\end{aligned}$
	& $ \gB_{\pi}^2 \xrightarrow{} \gB^2 \xrightarrow{} \gC^2$\\
	\hline
	SO(2) & $\gC_{\pi}:\{x\in \RR \,,\, -\pi \leq x \leq \pi \}$ 
	& $\begin{aligned}
        \theta = \arctan ({\mR[1,0]/ \mR[0,0]})
    \end{aligned}$ 
	& $\begin{aligned}
        \mR = \begin{bmatrix}
            \cos(\theta) & \sin(\theta) \\
             -\sin(\theta)& \cos(\theta) 
        \end{bmatrix} 
    \end{aligned}$ 
	& $\gC_{\pi} \xrightarrow{} \gC $\\
	\hline
	SO(3) & $\gB_{\pi}^3$ & $\begin{aligned}
	            \phi &= \arccos \left( \frac{1}{2} \left( \mathrm{Tr}(\mR) - 1 \right) \right) \\
            \vomega_{\textrm{x}} &= \frac{1}{2} \frac{\phi}{\sin \phi} \left( \mR - \mR^{\intercal} \right)
	\end{aligned}$
	& $\begin{aligned}
	        \phi &= \| \vomega \| \quad , \quad \hat{\vomega} = \vomega/ \phi \\
	                        \mR &=
                \cos \phi \mI+
                (1 - \cos \phi) \hat{\vomega}\hat{\vomega}^{\intercal} +
                \sin \phi \left[\hat{\vomega} \right]_{\textrm{x}}
	\end{aligned}$ 
	& $\gB^3_{\pi} \xrightarrow{} \gB^3 \xrightarrow{} \gC^3$\\
	\hline
	SE(2) & $\gC_{\pi}\times \RR^2$ &$\begin{aligned}
	        \mV = \frac{1}{\theta} \begin{bmatrix}
            \sin(\theta) & \cos(\theta) -1 \\
             1-\cos(\theta)& \sin(\theta)
        \end{bmatrix} \\
        \theta = \textrm{LogMap}(\mR)\quad,\quad \rho = \mV^{-1} \vt
	\end{aligned}$
	& $\begin{aligned}
	        \mV = \frac{1}{\theta} \begin{bmatrix}
            \sin(\theta) & \cos(\theta) -1 \\
             1-\cos(\theta)& \sin(\theta)
        \end{bmatrix} \\
        \mR = \textrm{ExpMap}(\theta)\quad,\quad \vt = \mV \rho
	\end{aligned}$
	& $\gC_{\pi}\times \RR^2 \xrightarrow{} \gC_{\pi}\times \gC_W^2 \xrightarrow{} \gC^3$\\
	\hline
	SE(3) & $\gB_{\pi}^3 \times \RR^3$& 
	$\begin{aligned}
	\mV = \mI + \left(\frac{1 - \cos(\phi)}{\phi^2}\right)\omega_{\textrm{x}} &+ \left(\frac{\phi - \sin(\phi)}{\phi^3}\right)\omega_{\textrm{x}}^2 \\
	\phi = \|\vomega\| \quad,\quad \vomega = \textrm{LogMap}(\mR) \quad &, \quad \rho = \mV^{-1} \vt
	\end{aligned}$ 
	& 	$\begin{aligned}
	\mV = \mI + \left(\frac{1 - \cos(\phi)}{\phi^2}\right)\omega_{\textrm{x}} &+ \left(\frac{\phi - \sin(\phi)}{\phi^3}\right)\omega_{\textrm{x}}^2 \\
	\mR = \textrm{ExpMap}{(\vomega)} \quad &, \quad \vt = \mV \rho
	\end{aligned}$ 
	& $\gB_{\pi}^3 \times \RR^3 \xrightarrow{} \gB^3 \times \gC_W^3 \xrightarrow{} \gC^6$\\
	\hline
\end{tabular}


==> tables/smooth_manifolds.tex <==
\begin{tabular}{ c | c | c | c | c | c} 
	\hline
	Manifold & $\hat{U}_{\gM}$ & LogMap & ExpMap & $\gamma$ & Adjoint Map\\
	\hline
	$\gS^2$ & $\gB_{\pi}^2:\{ \vx\in \RR^2 \,,\,  |\vx| \leq \pi \} $ & 
	$\begin{aligned}
    	\rho = \arctan\left(\frac{\sqrt{x^2 + y^2}}{z}\right) \quad ,& \quad \theta = \arctan\left(\frac{y}{x}\right) \\
    	 \hat{x} = \rho \cos(\theta) \quad ,& \quad  \hat{y} = \rho \sin(\theta)
	\end{aligned}$
	& 	$\begin{aligned}
	    \rho = \sqrt{\hat{x}^2 + \hat{y}^2} \quad ,& \quad
	    \theta = \arctan( \hat{y}/  \hat{x}) \\
	    x = \cos(\theta) \sin(\rho) \quad,\quad y &= \sin(\theta) \sin(\rho)\quad,\quad z = \cos(\rho)\\
	\end{aligned}$
	& $ \gB_{\pi}^2 \xrightarrow{} \gB^2 \xrightarrow{} \gC^2$
	& \\
	\hline
	SO(2) & $\gC_{\pi}:\{x\in \RR \,,\, -\pi \leq x \leq \pi \}$ 
	& $\begin{aligned}
        \theta = \arctan ({\mR[1,0]/ \mR[0,0]})
    \end{aligned}$ 
	& $\begin{aligned}
        \mR = \begin{bmatrix}
            \cos(\theta) & \sin(\theta) \\
             -\sin(\theta)& \cos(\theta) 
        \end{bmatrix} 
    \end{aligned}$ 
	& $\gC_{\pi} \xrightarrow{} \gC $ & 1\\
	\hline
	SO(3) & $\gB_{\pi}^3$ & $\begin{aligned}
	            \phi &= \arccos \left( \frac{1}{2} \left( \mathrm{Tr}(\mR) - 1 \right) \right) \\
            \vomega_{\textrm{x}} &= \frac{1}{2} \frac{\phi}{\sin \phi} \left( \mR - \mR^{\intercal} \right)
	\end{aligned}$
	& $\begin{aligned}
	        \phi &= \| \vomega \| \quad , \quad \hat{\vomega} = \vomega/ \phi \\
	                        \mR &=
                \cos \phi \mI+
                (1 - \cos \phi) \hat{\vomega}\hat{\vomega}^{\intercal} +
                \sin \phi \left[\hat{\vomega} \right]_{\textrm{x}}
	\end{aligned}$ 
	& $\gB^3_{\pi} \xrightarrow{} \gB^3 \xrightarrow{} \gC^3$ & $\mR_{\vx_0}^{\vx_1}$\\
	\hline
	SE(2) & $\gC_{\pi}\times \RR^2$ &$\begin{aligned}
	        \mV = \frac{1}{\theta} \begin{bmatrix}
            \sin(\theta) & \cos(\theta) -1 \\
             1-\cos(\theta)& \sin(\theta)
        \end{bmatrix} \\
        \theta = \textrm{LogMap}(\mR)\quad,\quad \rho = \mV^{-1} \vt
	\end{aligned}$
	& $\begin{aligned}
	        \mV = \frac{1}{\theta} \begin{bmatrix}
            \sin(\theta) & \cos(\theta) -1 \\
             1-\cos(\theta)& \sin(\theta)
        \end{bmatrix} \\
        \mR = \textrm{ExpMap}(\theta)\quad,\quad \vt = \mV \rho
	\end{aligned}$
	& $\gC_{\pi}\times \RR^2 \xrightarrow{} \gC_{\pi}\times \gC_W^2 \xrightarrow{} \gC^3$ & $\begin{aligned}
    \left(
        \begin{array}{c|c}
          \mR_{\vx_0}^{\vx_1} & [\vt_{\vx_0}^{\vx_1}]_\textrm{x} \mR_{\vx_0}^{\vx_1}\\
          \hline \mathbf{0} & \mR_{\vx_0}^{\vx_1}
        \end{array}
    \right)
	\end{aligned}$\\
	\hline
	SE(3) & $\gB_{\pi}^3 \times \RR^3$& 
	$\begin{aligned}
	\mV = \mI + \left(\frac{1 - \cos(\phi)}{\phi^2}\right)\omega_{\textrm{x}} &+ \left(\frac{\phi - \sin(\phi)}{\phi^3}\right)\omega_{\textrm{x}}^2 \\
	\vomega = \textrm{LogMap}{(\mR)} \quad &, \quad \rho = \mV^{-1} \vt
	\end{aligned}$ 
	& 	$\begin{aligned}
	\mV = \mI + \left(\frac{1 - \cos(\phi)}{\phi^2}\right)\omega_{\textrm{x}} &+ \left(\frac{\phi - \sin(\phi)}{\phi^3}\right)\omega_{\textrm{x}}^2 \\
	\mR = \textrm{ExpMap}{(\vomega)} \quad &, \quad \vt = \mV \rho
	\end{aligned}$ 
	& $\gB_{\pi}^3 \times \RR^3 \xrightarrow{} \gB^3 \times \gC_W^3 \xrightarrow{} \gC^6$ & $\begin{aligned}
    \left(
        \begin{array}{c|c}
          \mR_{\vx_0}^{\vx_1} & [\vt_{\vx_0}^{\vx_1}]_\textrm{x} \mR_{\vx_0}^{\vx_1}\\
          \hline \mathbf{0} & \mR_{\vx_0}^{\vx_1}
        \end{array}
    \right)
	\end{aligned}$\\
	\hline
\end{tabular}

